Event Representation with Sequential, Semi-Supervised Discrete Variables

Within the context of event modeling and understanding, we propose a new method for neural sequence modeling that takes partially-observed sequences of discrete, external knowledge into account. We construct a sequential neural variational autoencoder, which uses Gumbel-Softmax reparametrization within a carefully defined encoder, to allow for successful backpropagation during training. The core idea is to allow semi-supervised external discrete knowledge to guide, but not restrict, the variational latent parameters during training. Our experiments indicate that our approach not only outperforms multiple baselines and the state-of-the-art in narrative script induction, but also converges more quickly.

==> tables/tab_accf1.tex <==
\begin{table}[]
    \centering
    \scalebox{0.6}{
  \begin{tabular}{l|c|c|c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em} 
  \multirow{2}{*}{Model} & \multirow{2}{*}{$\epsilon$} & \multicolumn{3}{c|}{Valid} & \multicolumn{3}{c}{Test} \\ \cline{3-8} 
                         &                             & Acc   & Prec  & f1 & Acc   & Prec & f1 \\ \hline
                         RNNLM & - & 0.89   & 0.72 & 0.66 & 0.88  & 0.70  & 0.65 \\
                         RNNLM + ROLE  & - & \textbf{0.90}  & 0.78 & 0.73 & \textbf{0.89} & 0.77 & 0.71 \\ \cdashline{1-8}
                         Ours & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\ 
                         Ours & 0.20 & 0.66 & 0.23 & 0.22 & 0.67 & 0.23 & 0.22 \\ 
                         Ours & 0.40 & 0.76 & 0.34 & 0.33 & 0.76 & 0.34 & 0.32 \\ 
                         Ours & 0.50 & 0.78 & 0.42 & 0.39 & 0.78 & 0.41 & 0.38 \\ 
                         Ours & 0.70 & 0.84 & 0.64 & 0.61 & 0.83 & 0.63 & 0.61 \\
                         % chain & 0.80 & 0.85 & 0.85 & 0.70 & 0.85 & 0.68 & 0.84 & 0.84 & 0.72 & 0.84 & 0.69 \\
                         % chain & 0.90 & 0.86 & 0.86 & 0.77 & 0.86 & 0.75 & 0.86 & 0.86 & 0.77 & 0.86 & 0.76 \\ \hline
                         Ours & 0.80 & 0.86 & 0.75 & 0.74 & 0.85 & 0.75 & 0.75 \\
                         Ours & 0.90 & 0.87 & \textbf{0.81} &   \textbf{0.79}   &  0.87 &    \textbf{0.81}  &   \textbf{0.79} \\                       
  \specialrule{.1em}{.05em}{.05em} 
  \end{tabular}
  }
  \caption{Accuracy, and macro precision and F1-score.}
  \label{table:acc}
\end{table}

==> tables/tab_intro_infer_examples.tex <==
\begin{table*}[]
\label{tab:intro_infer_frames}
\begin{subtable}[t]{.5\textwidth}
\centering
\scalebox{0.62}{  
\begin{tabular}{l|l|l|l}
\specialrule{.1em}{.05em}{.05em} 
\multicolumn{2}{c|}{Event} & Ground Truth& Inferred Frame ($f$) \\ \hline
1 &   she competed in olympics & \fsc{\blue{Win_prize}} & \fsc{{Win_prize}} \\ \hline
2 &  she set at championships & \fsc{\blue{Cause_to_start}} & \fsc{{Cause_to_start}} \\ \hline
3 &  she named in <unk>& \fsc{\orange{Appointing}} & \fsc{{Being_named}} \\ \hline
4 &  she started but had& \fsc{\orange{Process_start}} & \fsc{{Activity_start}} \\ \hline
5 & they had because_of height & \fsc{\blue{Possession}} & \fsc{{Possession}} \\ 
\specialrule{.1em}{.05em}{.05em} 
\end{tabular}
}
\caption{Example (Training)}
\label{tab:intro_infer_train}
\end{subtable}
~
\begin{subtable}[t]{.5\textwidth}
\centering
\scalebox{0.62}{  
\begin{tabular}{l|l|l|l}
\specialrule{.1em}{.05em}{.05em} 
\multicolumn{2}{c|}{Event} & Ground Truth& Inferred Frame ($f$)\\ \hline
1 & it features in form& \fsc{\orange{Inclusion}} & \fsc{{Inclusion}} \\ \hline
2 & format allows and provides & \fsc{\orange{Permitting}} & \fsc{{Deny_permission}} \\ \hline
3 & format provides none forum & \fsc{\orange{Supply}} & \fsc{{Supply}} \\ \hline
4 & readers rely upon staff & \fsc{\orange{Reliance}} & \fsc{{Reliance}} \\ \hline
5 & citations support none assertions& \fsc{\orange{Supporting}} & \fsc{{Taking_sides}} \\
\specialrule{.1em}{.05em}{.05em} 
\end{tabular}
}
\caption{Example (Validation)}
\label{tab:intro_infer_val}
\end{subtable}
\caption{Sequences of 5 events and the inferred frames during training with partial frame observation, and validation without any observation. Blue frames are observed and orange frames are latent.}
\label{tab:infer-examples-train-val} 
\end{table*}

==> tables/tab_invNarrCloze.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.72}{ 
    \begin{tabular}{l|c|c|c|c|ccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{1}{|c|}{\multirow{3}{*}{$\epsilon$}}  & \multicolumn{4}{|c}{Inv Narr Cloze} \\ \cline{3-6} 
    \multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{}  & \multicolumn{2}{|c|}{Wiki} & \multicolumn{2}{|c}{NYT} \\ \cline{3-8} 
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & Valid & Test & Valid & Test \\ \hline
     RNNLM & -    &     20.33       &      20.44       & 17.65   &  17.45 \\ 
     RNNLM+ROLE & -     &      20.32       &       20.18       &  17.60   &   18.20 \\ 
     HAQAE & - & 27.80 & 26.05 & 20.15 & 22.35 \\ \cdashline{1-6}
     Ours & 0.0  & 37.00 & 43.00 & 28.70 & 28.25 \\ 
     Ours & 0.2 & \textbf{47.50} & \textbf{48.55}& \textbf{30.45} & 29.40 \\ 
     Ours & 0.4  & 43.75 & 43.75 & 28.75 & 30.40 \\ 
     Ours & 0.5  & 40.25 & 39.45 & 27.90 & 29.20 \\ 
     Ours & 0.7 & 38.00 & 40.85 & 30.05 & \textbf{30.70} \\ 
     Ours & 0.8  & 37.15 & 36.75 & 29.15 & 29.40 \\ 
     Ours & 0.9  & 35.95 & 36.45 & 30.00 & 29.60 \\
    \specialrule{.1em}{.05em}{.05em} 
    \end{tabular}
    }
    \caption{Inverse Narrative Cloze scores (higher is better), using 500 frames and 5 clauses. %
    All of the models are trained with Wiki and then tested on either Wiki or NYT as appropriate.} 
    \label{tab:invNarrCloze}
\end{table}

==> tables/tab_invNarrCloze_wostats.tex <==
\begin{subtable}[t]{.53\textwidth}
    \centering
    \scalebox{0.6}{ 
    \begin{tabular}{l|c|c|c|c|ccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{1}{|c|}{\multirow{3}{*}{$ \epsilon $}}  & \multicolumn{4}{|c}{Inv Narr Cloze} \\ \cline{3-6} 
    \multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{}  & \multicolumn{2}{|c|}{Wiki} & \multicolumn{2}{|c}{NYT} \\ \cline{3-8} 
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & Valid & Test & Valid & Test \\ \hline
     RNNLM       & -  
     & 20.33  
     &  21.37 
     & 18.11 
     & 17.86 
     \\ 
     RNNLM+ROLE  & -  
     & 19.57 
     & 19.69 
     & 17.56 
     & 17.95 
     \\ 
     HAQAE       & -  
     & 29.18 
     &  24.88 
     & 20.5 
     & 22.11 
     \\ \cdashline{1-6}
     Ours & 0.0  
     &  43.80 
     & 45.75 
     & 29.40 
     & 28.63 
     \\ 
     Ours & 0.2  
     &  45.78 
     &  44.38 
     & 	29.50 
     &  29.30 
     \\ 
     Ours & 0.4  
     &  \textbf{47.65} 
     & 	\textbf{47.88} 
     &  \textbf{30.01} 
     &  \textbf{30.61} 
     \\ 
     Ours & 0.5  
     &  42.38 
     &  40.18 
     &  29.36 
     &  29.95 
     \\ 
     Ours & 0.7  
     & 38.40 
     & 39.08 
     & 29.15 
     & 30.13 
     \\ 
     Ours & 0.8  
     & 	39.48 
     & 	38.96 
     &  29.50 
     &  30.33 
     \\ 
     Ours & 0.9  
     &  35.61 
     &  35.56 
     &  28.41 
     &  29.01 
     \\
    \specialrule{.1em}{.05em}{.05em} 
    \end{tabular}
    }
    \caption{Inverse Narrative Cloze scores (higher is better), using 500 frames and 5 clauses. %
    All of the models are trained with Wiki and then tested on either Wiki or NYT as appropriate.
    Due to space constraints, we present standard deviations in \cref{tab:invNarrClozeStats}.
    } 
    \label{tab:invNarrClozewostats}
\end{subtable}

==> tables/tab_nonverb_clusters.tex <==
  \begin{table*}[!ht]
    \centering
    \resizebox{.98\textwidth}{!}{
    \begin{tabular}{l|ccccc}
    \specialrule{.1em}{.05em}{.05em} 
     {Non-Verbs}& \multicolumn{5}{c}{$\beta_{\text{enc}}$ (\textbf{\fsc{Frames} Given Verbs})} \\ \cdashline{1-6}
    \textbf{chairman} & \fsc{Assistance} & \fsc{Volubility} & \fsc{Supply} & \fsc{Change_of_leadership} & \fsc{Successfully_communicate_message} \\ 
    \textbf{licence} & \fsc{Grant_permission} & \fsc{Permitting} & \fsc{Activity_stop} & \fsc{Commerce_buy} & \fsc{Commerce_sell} \\ 
    \textbf{business} & \fsc{Commerce_pay} & \fsc{Commerce_buy} & \fsc{Expensiveness} & \fsc{Renting} & \fsc{Reporting} \\ 
    \textbf{company} & \fsc{Assistance} & \fsc{Range} & \fsc{Supply} & \fsc{Employing} & \fsc{Commerce_buy}\\
    \textbf{paper} & \fsc{Submitting_documents} & \fsc{Summarizing} & \fsc{Sign} & \fsc{Deciding} & \fsc{Explaining_the_facts}\\
    \textbf{authority} & \fsc{Leadership} & \fsc{Justifying} & \fsc{Clarity_of_resolution} & \fsc{Commitment} & \fsc{Interrupt_process}\\
    \specialrule{.1em}{.05em}{.05em}     
    \end{tabular}
    }
\caption{Results for the outputs of the attention layer, the upper table shows the $\beta_{\text{enc}}$ and the bottom table shows the $\beta_{\text{dec}}$, when $\epsilon=0.7$. Each row shows the top 5 words for each clustering. 
See \cref{tab:moreClusters} in the Appendix.
}
\label{tab:attentionNonVerbClusters}
\end{table*} 

==> tables/tab_ppx.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l|c|c|c}
    
    \specialrule{.1em}{.1em}{0.01em}
    \multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{1}{|c|}{\multirow{3}{*}
    {$\epsilon$}
    % {\scalebox{5}{$\epsilon}$}}
    } & \multicolumn{2}{|c}{PPL} \\
    \cline{3-4} 
    % \cline{3-4} 
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & Valid & Test  \\ \hline
    RNNLM & - &  62.79    &   61.67    \\ 
    % \hline
     RNNLM+ROLE & - & 66.36    &    64.46    \\ 
    %  \hline
    HAQAE & - & 24.92 & 21.68 \\ \cdashline{1-4}
    % \hline
    Ours & 0.0 & 40.34 & 36.76  \\ 
    % \hline
    Ours & 0.2 & 38.03 & 33.34  \\ 
    % \hline
    Ours & 0.4 & 37.90 & 33.45 \\ 
    % \hline
    Ours & 0.5 & 36.06 & 31.47 \\ 
    % \hline
    Ours & 0.7 & 23.09 & 20.38 \\ 
    % \hline
    Ours & 0.8 & 22.83 & 19.97 \\ 
    % \hline
    Ours & 0.9 & \textbf{22.17} & \textbf{19.45} \\
    \specialrule{.1em}{.1em}{0.005em}
\end{tabular}
    \caption{Validation and test per-word perplexities (lower is better).  %
    Recall that $\epsilon$ is the (average) percent of frames observed during \textit{training} though during evaluation \textit{no} frames are observed. %
    We always outperform RNNLM and RNNLM+ROLE, and outperform HAQAE when automatically extracted frames are sufficiently available during training ($\epsilon \in \{0.7, 0.8, 0.9\}$). %
    }
    \label{tab:Perplexity}
\end{table}
